Standardization of Cloth Objects and its Relevance in Robotic Manipulation

The field of robotics faces inherent challenges in manipulating deformable objects, particularly in understanding and standardising fabric properties like elasticity, stiffness, and friction. While the significance of these properties is evident in the realm of cloth manipulation, accurately categorising and comprehending them in real-world applications remains elusive. This study sets out to address two primary objectives: (1) to provide a framework suitable for robotics applications to characterise cloth objects, and (2) to study how these properties influence robotic manipulation tasks. Our preliminary results validate the framework's ability to characterise cloth properties and compare cloth sets, and reveal the influence that different properties have on the outcome of five manipulation primitives. We believe that, in general, results on the manipulation of clothes should be reported along with a better description of the garments used in the evaluation. This paper proposes a set of these measures.

==> sections/Evaluation.tex <==
\begin{wrap}

\section{Evaluation}\label{sec:radarchart} % Radar chart / cloth sets

In this section we want to present the usage of the presented methods. It should be divided into two sections: the first one focused on demonstrating the use of radar chart to compare different cloth sets found in literature, and the second one to show which type of cloth set should be used, based on the shape the radar chart, according to the tackled task.

\begin{itemize}
    \item \sout{Purpose and meaning of the radar chart. How to report cloth sets? How to use it as visual a comparison.}
    \item \sout{Generation of the radar chart. Join measures from section \ref{sec:properties} + physical properties.} This will be explained in Section \ref{sec:properties}.
\end{itemize}


\begin{itemize}
    \item Show radar chart of different cloth sets. Explain the differences, the advantages and disadvantages of each, the suitability for its purpose (or the shape that it should have), for what applications would be interesting to be used.
    \item Relate the results of the primitives with the results of the radar chart. Plot a line graphic that show the values of the measurement systems and of the primitives evaluations of each property for each selected sample (it should have the same tendency: low extreme, medium, high extreme). Demonstration that through interaction (with simple actions) it is possible to identify cloth parameters. 
\end{itemize}
    
\subsection{Comparison between existing cloth sets}

\begin{itemize}
    \item Section to validate utility of the radar chart..
    \item Analysis of resulting radar charts of different cloth sets found in literature (through visual comparison). What do they represent? What are they providing? Should they be different?
\end{itemize}

\subsection{Primitives result} %Not this title


%Property identification through interaction

Explain what type of radar chart is necessary to have according to the application (using results from Section \ref{sec:primitives}).

\end{wrap}
